GlucoAgent: Personalized Glucose Forecasting from Multimodal Personal Context

Continuous glucose monitors, smartwatches, meal logs, and health profiles form a rich multimodal personal context that can significantly enhance glucose forecasting. However, existing methods struggle to effectively utilize these signals to improve glucose prediction because the relevance of different modalities varies drastically across individuals and time. We present GlucoAgent, an LLM-based agentic system that addresses this challenge through dynamic, case-by-case analysis at inference time. For each forecast, GlucoAgent writes and runs code over an individual's multimodal context and returns predictions with a reason and supporting evidence. The generated programs are highly diverse, ranging from retrieving similar past meals to fitting and back-testing physiological and statistical models. On CGMacros, a multimodal glucose dataset, GlucoAgent outperforms time series foundation models on every forecasting horizon, achieving an average RMSE of 22.5 mg/dL compared to 23.5 mg/dL of Chronos-2, the leading multimodal time series foundation model. Furthermore, GlucoAgent is highly effective at leveraging multimodal data. The addition of multimodal data reduces its average RMSE by 1.4 mg/dL (24.0 mg/dL to 22.5 mg/dL), compared to a marginal 0.3 mg/dL (23.8 mg/dL to 23.5 mg/dL) improvement for Chronos-2. This advantage is most pronounced in challenging post-meal windows, where GlucoAgent uses multimodal context to reduce 60-minute forecast RMSE by 4.6 mg/dL (31.0 mg/dL to 26.5 mg/dL), far exceeding the 0.8 mg/dL (31.9 mg/dL to 31.1 mg/dL) reduction achieved by Chronos-2.

==> GenAI4H/preamble/macros.tex <==

\newcommand{\agentname}{GlucoAgent}              %
\newcommand{\Agentname}{GlucoAgent}              %
\newcommand{\agentnameposs}{GlucoAgent's}        %

\newcommand{\agentmm}{the multimodal configuration}
\newcommand{\Agentmm}{The multimodal configuration}
\newcommand{\agentcgm}{the glucose-only configuration}
\newcommand{\Agentcgm}{The glucose-only configuration}


\newcommand{\llmgeneric}{a general-purpose frontier large language model}
\newcommand{\Llmgeneric}{A general-purpose frontier large language model}
\newcommand{\llmexact}{Claude Opus~5}
\newcommand{\llmexactid}{\texttt{us.anthropic.claude-opus-5}}

\newcommand{\maxturns}{16}          %
\newcommand{\maxcodecalls}{14}      %
\newcommand{\maxouttokens}{6{,}144} %
\newcommand{\sandboxtimeout}{8}     %
\newcommand{\sandboxmem}{512}       %
\newcommand{\maxcodebytes}{48{,}000}%
\newcommand{\maxcapturebytes}{32{,}000} %

\RequirePackage[T1]{fontenc} %
\RequirePackage{booktabs}    %
\RequirePackage{fvextra}     %
\newcommand{\xin}[1]{\textcolor{red}{[XS: #1]}}

